Time Constrained Continuous Subgraph Search over Streaming Graphs

The growing popularity of dynamic applications such as social networks provides a promising way to detect valuable information in real time. Efficient analysis over high-speed data from dynamic applications is of great significance. Data from these dynamic applications can be easily modeled as streaming graph. In this paper, we study the subgraph (isomorphism) search over streaming graph data that obeys timing order constraints over the occurrence of edges in the stream. We propose a data structure and algorithm to efficiently answer subgraph search and introduce optimizations to greatly reduce the space cost, and propose concurrency management to improve system throughput. Extensive experiments on real network traffic data and synthetic social streaming data confirms the efficiency and effectiveness of our solution.

==> maintenance.tex <==
\section{Maintenance}
\nop{
\begin{enumerate}
\item 
	Register expired time for all deletion.
\item
	Candidate list.
\end{enumerate}
}


Under this model, maintenance of our index must be considered. When a new edge $e_t$ comes into the time window (i.e. an insertion operation), if $e_t$ matches at least one query edge, then our index, including the one-step join and all maps, may be outdated and need to be updated. Besides, if an edge in our index expires from the time window(i.e. a deletion operation), our index need to be updated as well. We will discuss how to update our index for insertion and deletion, respectively. Since it is trivial to maintain each candidate list and the one-step join result, we do not consider the maintenance of them when insertion or deletion happens. Instead, we focus on the maintenance of the map $F_{e_i}$ for each trigger edge $e_i$ in $Q$.

\subsection{Insertion}
\subsubsection{Pruning}


%First reduce
Now, let's discuss the maintenance of the core index: $F_{e_i}$, where $e_i$ is a trigger edge of $Q$. Assuming that an edge $e_t = (v_a, v_b)$ comes and $e_t$ matches $e_q = (a, b)$. Note that $e_t$ may match more than one edge in the query $Q$ and we only discuss one of them for presentation simplicity only. We know that for a trigger edge $e_i$, each key in $F_{e_i}$ is a match of subquery $\N^-(e_i)$ and each value is a list consisting of items who are matches of subquery $Q\setminus \N(e_i)$. Thus, $F_{e_i}$ may be outdated only if the coming edge $e_t$ matches one of the query edge in $Q\setminus \Gamma(e_i)$, namely, $\qminusi$. Formally, we have the following lemma.
\begin{lemma}
Consider an edge $e_t$ matching $e_q \in Q$ comes in to the time window. For each trigger edge $e_i$, if $e_q \in \Gamma(e_i)$, namely, $e_q$ is a edge adjacent to $e_i^s$ or $e_i^t$, then $F_{e_i}$ does not need to be updated.
\end{lemma}
\nop{ % Put in proof
Note that, for an incoming edge $e_t$ who matches a trigger edge $e_q$, $e_t$ may incur a new match $s$ for $Q$ while since 
}

%Second reduce
Let's consider the case when an edge $e_t$ matching $e_q \in \qminusi$ where $e_i$ is a trigger edge in $Q$. According to the definition of $F_{e_i}$, for each pair $(s_k, s_v)$ where $s_k$ is a match of subquery $\N^-(e_i)$ and $s_v$ is a item in the corresponding value list $F_{e_i}(s_k)$, $s_k \cup$ $s_v$ is exactly a match of $\qminusi$. Thus, $F_{e_i}$ needs to be updated for $e_t$ only if there is a new pair $(s_{k'}, s_{v'})$ incurred by $e_t$ to be added into $F_{e_i}$, where $s_{k'} \cup$ $s_{v'}$ is a new match of $\qminusi$ in the time window. Recall Lemma \ref{lem:triggermatch}, we can know that $F_{e_i}$ need to be updated only if $e_q$ is a trigger edge of subquery $\qminusi$. 

\begin{lemma}\label{lem:triggerupdate}
Given a new edge $e_t$ matching $e_q$ in $Q$,  for each trigger edge $e_{i} \in Q$ where $e_{q} \in \qminusi$,
if $e_q$ is not a trigger edge of $\qminusi$, then $F_{e_{i}}$ does not need to be updated.
\end{lemma}

According to Lemma \ref{lem:triggermatch} and Lemma \ref{lem:triggerupdate}, for an coming edge $e_t$ who matches $e_q$, we only consider the update of $F_{e_i}$ if $e_q$ is an trigger edge of subquery $\qminusi$.

\subsubsection{Update \large $F_{e_i}$}
Let's discuss the case when the update of $F_{e_i}$ is inevitable, namely, a coming edge incur at least a new match of subquery $\qminusi$. The straightforward method is to conduct subgraph isomorphism search starting from the coming edge and figure out all new matches for $\qminusi$, which is obviously too time-consuming. We will discuss some optimization to accelerate the update of each map $F_{e_i}$.

For a trigger edge $e_i$ in $Q$, consider the subquery formed by deleting $\Gamma(e_i)$ from $Q$, namely, $\qminusi$. Although $Q$ is connected as we assume, $\qminusi$ may be disconnected. For example in Figure \ref{fig:mapschema:e4}, we can see that after deleting \{$d$, $c$\} from query $Q$, the remaining query graph is a disconnected graph with two connected components:\{$a, b$\} and \{$e, f$\}. Maintaining all matches for a disconnected subquery is costly on both time and space. Specifically, we assume that there are $m$ connected components in $\qminusi$: \{$C_1$, $C_2$,$\cdots$, $C_m$\}. Then the set of matches for subquery $\qminusi$, denoted as $M(\qminusi)$, will be as following:
\[M(\qminusi) = M(C_1)\times M(C_2)\times \cdots M(C_m)\]
Thus, storing the whole $M(\qminusi)$ costs too much space. Instead, we just maintain matches for each $C_{m'}$ ($1\leq m' \leq m$) and the space we cost for these matches is hugely reduced to 
\[M(C_1) + M(C_2) + \cdots M(C_m)\]

We can see that maintenance of different connected components of $\qminusi$ is independent with each other. Without loss of generality, we only discuss the maintenance of the connected component $C_1$ in $\qminusi$. Recursively, we can see that maintenance of $C_1$ in the graph stream $G$ over time window $W$ is exactly the problem $\phi(G, W, C_1)$.
However, the size of $C_1$ may just be much smaller than query $Q$ and problem $\phi(G, W, C_1)$ may be solved in a direct way. For example, consider the map of trigger edge $e_4 = (d, c)$. When we delete $d$ and $c$ from query $Q$, each of the remaining two connected components contain only one single edge: $C_1=$ \{$a, b$\} and $C_2$ = \{$e, f$\}. Thus, $\phi(G, W, C_1)$ corresponds to all matches of edge $e_1=$ $(a, b)$, which is exactly the candidate list of $e_1$, namely, $CL(e_1)$. Specifically, we will discuss the how to solve the $\phi(G, W, C_1)$ regarding the size of $C_1$. In fact, all these discussions are absolutely applied to $\phi(G, W, Q)$ and we do not discuss this at the most beginning for just presentation reason only.

\begin{enumerate}
\item 
	If $|C_1|=1$, we can just remove $C_1$ from the key schema of the $F_{e_i}$ because there is nothing to do with $C_1$ on the maintenance of $F_{e_i}$. Besides, since $C_1$ contains only a vertex who is a neighbor of $e_i^s$ or $e_i^t$, then when edge $e_t$ comes, all matches of $C_1$ can easily be figured out over the one-step join result of $e_t$.
\item
	If $|C_1|=2$, $C_1$ contains a single edge and all matches of $C_1$ are exactly in the corresponding candidate list of the edge in $C_1$.
\item 
	If $|C_1| > 2$, we will recursively solve $\phi(G, W, C_1)$ by maintaining corresponding maps, as what we do for $\phi(G, W, Q)$.

\end{enumerate}





\subsection{Deletion}
It is non-trivial to delete expired records to update the index.  

For the candidate lists, since they are sorted in time order. When an edge is expired, the edge must be the oldest one in the list and we can just remove the edge from the list and update the neighbor information of neighbors of this edge.

\textbf{Expiring List.}

For the KV-index, if a key expired, (i.e. a key containing an expired edge), since the key set is not sorted in chronological order, removing expired keys may not be so straightforward. In fact the expired time of a key is exactly the minimum timestamp of edges in the key, which is immediately determined at creating of this key. Thus, when a key is first added into the index, we ``register'' this key to its edge of minimum timestamp. Specifically, we keep a inverted list for each edge in the graph stream and each item in this list is the key containing this edge as the one of minimum timestamp. When a key is first created, we can easily append the key into the list of the edge with minimum timestamp in this key. When an edge expired, we can search each key in the corresponding list and remove those key from the index. Similarly, we can also add each value item in this list (Define this list as a expiring list) and remove the value item when this edge expire. Note that, when the key is removed, the corresponding value is also removed and corresponding expiring list is updated.

****Figure presents.


Considerations for $F_{e_i}$
\begin{enumerate}
\item
	If $e_q \in \Gamma(e_i)$, then $F_{e_i}$ should not be adjusted since $e_q$ is neither in key schema nor in value schema of $F_{e_i}$.
\item
	$F_{e_i}$ needs to be updated only if $e_q$ is an edge in $Q\setminus \Gamma(e_i)$.
\item
	Computation is huge, 
	\begin{enumerate}
	\item 	Reduce: discuss $F_{e_i}$ when it is disconnected. Maintain them separately.
		
	\item 	repeated connected component. 
		
	\item 	Cost Model: recursive, consider the case recursion incurring overlap.  Why not consider cost model at the initial stage.
		
	\item 	Given two edge $e_1$, $e_2$, consider the relationship between their corresponding map $F$. If both $e_1$ and $e_2$ are trigger edges, then if $e_t$ match $e_1$, we have compute $subN(e_t)$. And hopefully, $subN(e_t)$ can play an important role in updating $F_{e_2}$.
	
	\item   Each trigger edge is taken care by its corresponding map.  The latency of newly-match for $Q$ is much important than its subquery.
	\end{enumerate}	
\end{enumerate}



\subsubsection{Candidate List}



\nop{
However, if we keep each map up to date, we need to  update $|E_q|-1$ maps when an update of edges in the time window happen, which is very time consuming. Besides, we may also wastefully bring in lots of key-value pairs that will never used to constitute a matching result of given query. (maybe some also not constitute, but inevitable)

Thus, we maintain these maps in an \textbf{latent} way. In fact, we do not keep these maps up to date and instead, we just use these map to record corresponding key-value pairs that is produced previously. In detail, when a edge $e_t = (v_a, v_b)$ matching $e_q = (a, b)$ (Assuming that $e_q$ has no IN timing edge) comes into time window, we assume that $M(v_a, v_b)$ are the set of matching results of subquery $\N(a, b)\cup\{a,b\}$ arise from $(v_a, a_j)$ . For each matching result $s$ $\in M(v_a, v_b)$, our target is to figure out all newly matching of $Q$ containing $s$, with the help of the maps. Assuming that $s'$ is a complementary part of $s$ in a newly matching of $Q$, namely, $s' \cup s$ $\in M(Q)$. There are two case for $s'$. The first case is that $s'$ may be found in the value list of key $s$ searching map $Map(e_q)$. And the other case is that $s'$ is not in outdated $Map(e_q)$ and we explore $s' \cup s$ starting from $s$ over the candidate lists and update $Map(e_q)$. For the second case, since there are already some value items of key $s$, we design our exploration to avoid repeatedly computing them. 

**** Value should not be a list , it could be a DAG.
}


\nop{
\section{Previous}
We know that each update is so local that it incurs only minor change of all edges in the time window and there are still lots of overlapping intermediate results between two calls of SGI algorithm for two consecutive coming edges in graph stream. For example, given query $Q_0$, assuming that $e_{t_i}$ and $e_{t_j}$ ($t_i$ $< t_j$) are two consecutive edges who match $e_3$ and $e_4$, respectively. The SGI starting from $e_{t_i}$ and that starting from $e_{t_j}$ share lots of intermediate results, most of which is the isomorphic subgraphs of induced subgraph over \{$e_1$, $e_2$, $e_4$, $e_5$\} $\subset$ $E_q$. Thus, when we conduct the SGI algorithm for $e_{t_i}$, the computation results over \{$e_1$, $e_2$, $e_5$\} can be utilized to speed up the SGI algorithm for $e_{t_j}$. For convenience, given a subquery $g$ of $Q$, we use $M(g)$ to denote the set of matching results of $g$ over the edges in time window. Details of these two operation will be discussed later and for complementing subgraph in $subN(v_a, v_b)$, we assume that there is a black box index $I$ which will return all possible matching subgraphs of $Q$ containing $(v_a, v_b)$ when inputted with $subN(v_a, v_b)$. 

Given a coming edge $e_t$ where $e_t$ matches $e_q$ $\in E_q$, $e_t$ will result in newly matching subgraphs only if there is no such $e_p$ $\in E_q$ where $e_q$ $\prec e_p$. Hence, we only consider the case that newly matching subgraphs may appear. Take a coming edge $e_t$ who matches $e_3$ $\in E_q$ for example. Since there is no other edge in $E_q$ that is required to come before $e_3$, we assume that $m = $ \{$e_{t_1}$, $e_{t_2}$, $e_{t}$, $e_{t_4}$, $e_{t_5}$\} is a newly matching subgraphs. We can see that edges of direct relation with $e_3$ are only $e_2$ and $e_5$. Thus, before finding $m$, we need inevitably to figure out adjacent comparable edges of $e_t$ in graph stream. And it is easy to understand that the least inevitable computation to find $m$ is to find out \{$e_{t_2}$, $e_{t}$, $e_{t_5}$\} which is a matching result of \{$e_2$, $e_3$, $e_5$\} since \{$e_{t_1}$, $e_{t_2}$, $e_{t_4}$, $e_{t_5}$\} may probably have been found as a matching result of \{$e_1$, $e_2$, $e_4$, $e_5$\} during previous exploration starting from an edge who also matched $e_3$. In other words, when $e_t$ who matches $e_3$ comes, we hope that we need only to find the matching results of the subquery made up of $e_3$ and its adjacent edges in $E_q$ where the matching results will be further extended into matching subgraphs by being merged with previous matching results of the complement of that subquery, namely, \{$e_1$, $e_4$\}.

Specifically, for each edge $e_q = (a, b)$ $\in E_q$, we maintain a map where the keys are some matching results of $\N^-(a, b)$, namely, a subset of $M(\N^-(a, b))$.
 While the corresponding value of a specific key $g_k$ is a list of subgraphs in the graph stream: \{$g_{v_1}$, $g_{v_2}$,...,$g_{v_k}$\} where $g_k$ $\cup g_{v_k'}$ ($1 \leq k' \leq k$) is a matching result of $Q\setminus$ $\{a, b\}$. We denote the map of $e_q$ as $F_{e_q}$.
Formally:
\[F_{(a,b)}:\;\;\N^-(a,b) \rightarrow Q\setminus\N(a,b)\]
 
For example, the corresponding map of each edge in $Q_0$ is presented as follows:
	\begin{itemize}
		\item
			$e_1 = $ ($a, b$): \{$c$, $d$\} $\rightarrow$ $\{e\}$
		\item 
			$e_2 = $ ($b, c$): \{$a$, $d$, $e$\} $\rightarrow$ $\emptyset$
		\item
			$e_3 = $ ($a, c$): \{$b$, $e$\} $\rightarrow$ $\{d\}$
		\item
			$e_4 = $ ($b, d$): \{$a$, $c$\} $\rightarrow$ $\{e\}$
		\item
			$e_5 = $ ($c, e$): \{$a$, $b$\} $\rightarrow$ $\{d\}$
	\end{itemize}

Note that, for some edge $e_q = (a, b)$ in $E_q$, when deleting $e_q$ from the corresponding query $Q$, the origin query may decompose into two(At most) separate connected subquery. (..., for example). Thus, it is beneficial on both time and space to attaches two maps for each edge of this kind. Since two maps are structurally independent to each other, we can maintain each map independently. For simplicity, we only discuss that there is only a map for each edge.

With these maps, when an edge $e_t = (v_a, v_b)$ matching $e_q$ $= (a, b)$ $\in E_q$ comes, the computation of the query can be improved as follows:
\begin{enumerate}
\item 
	We first compute the $M(\N(v_a, v_b))$. The computation is trivial since any two edges in subquery  $\N(v_a, v_b)$ are either adjacent directly or having common adjacent edge, i.e. $e_t$\footnote{Further optimization remains to be discussed}.
\item
	We use $\Phi(v_a, v_b)$ denotes the set formed by projecting $M(\N(v_a, v_b))$ over $\N^-(v_a, v_b)$, namely,
	\[\Phi(a, b) = \Pi_{\N^-(a, b)}(M(\N(a, b)))\]
	For each subgraph $s$ in $\Phi(v_a, v_b))$, we search the value list\footnote{Maybe there is a better data structure (Maybe not)} in the map $F_{e_q}$ with $s$ as a key. Then, for each $s'$ in the value list, subgraph $s\oplus s'\oplus \{v_a, v_b\}$ must be a matching subgraph\footnote{Note that timing constraint has already been addressed since $(v_a, v_b)$ must be the newest.}. 
\end{enumerate}

We can see that, computation of $M(Q)$ and verification is reduced into that of $M(\N(a, b))$ added to that of searching on the $Map(e_q)$. Obviously, the reduction is highly considerable.




\section{Previous Draft2}
*** outdated label is not so effective.

\begin{enumerate}
\item 
	We first compute the $\trans{SGI}(\{e_q\cup \N(e_q)\})$. It is easy since any two edges in subquery  $\{e_q\cup \N(e_q)\}$ are either adjacent directly or having common adjacent edge, i.e. $e_t$.(The same as previous first step)
\item
	We keep record a status of each maps, if the coming edge is possible to incur adjustment of a certain map, we set the map as outdated. (consider how to deal with deletion of edge)
\item
	If $Map(e_q)$ is not outdated, find a way to efficiently compute newly matchings (may be we don't need to conduct the first step when key set is not large, or may be we should reduce the range of the first step according to the key set. Maybe these two ideas are of no sense). 
\end{enumerate}

**** It seems that, concept of "outdated" is of no sense if we don't keep map up to date all the time. Only keys adjacent of previously coming edges will exist in the map key set and those keys conforming with subsequent coming edges may just not exist in the map.

**** It is important to notice that for each edge $e_q$, its two vertexes $e_{q}^s$ and $e_{q}^t$ are the linked part to other adjacent edges. Sometimes, all adjacent edges link to only one vertexes of $e_q$, and the key should be just the two vertexes of an edge matching $e_q$. However, for an edge $e_t$ $= (a, b)$ matching $e_q$, the matching result of $\{e_q\cup \N(e_q) \}$ which contains $e_t$ is more than one while all these matching results(keys) can be grouped in the same segment. \textbf{Basing} on this thoughts, let's think about when the keys will be used. We know that each key is a partial matching result, thus, each key exactly corresponds to a pair of vertexes, namely, a key created when $(a, b)$ comes, will be used only when $(a, b)$ comes again(May be wrong). Think about the two linkage and determine what constitute a map!!
\begin{enumerate}
\item 
	Linkage from a coming edge to the key is a nonempty subset of \{$(a, b)$\}, where $a$ and $b$ are two vertexes of the coming edge.
\item
	Linkage from a key to a value tuple is also a nonempty set of vertexes who are exactly the overlapping vertexes between key edges and value tuple.
\end{enumerate}
So, with these thoughts, we should not consider the map over the ``Together'' query, instead, \textbf{maybe} we should just focus on the structural graph. We may impose timing order to do some optimization, of course.

1. Continue to think about when key will be used!!  use ratio of the keys
More significant optimization must be found!!!
2. reduce the time computing initial SGI?
3. reduce the time searching maps?
utilizing timing feature?

**** For an matching result of the value, there are two cases:
 one is that this result is never figured out before. In this case, we need to compute it for the first time. The other is that this result is ever figured out during last computation when an edge which also matches $e_q$ came into the time window. In this second case, we know that it must be available in the corresponding map and easy to figure out. 






\begin{algorithm}[t]
\small
\caption{Insertion}
 \label{alg:insertion}
\KwIn{A new edge $e_t$ in $E$ at time $t$}
\KwOut{Updated Hyper Graph $\trans{G}$}
Compute $Match(e_t)$ as the set of edges which $e_t$ matches in $E_q$ \\
\If{$Match(e_t) = \emptyset$}{RETURN}
Add $e_t$ into $\trans{V}$ as a vertex  \\
Compute $\trans{N}(e_t) = \{v(e') \in \trans{V}\ |\ e' \cap e_t \neq \emptyset\}$. \\

\ForEach{$e_{t'} \in \trans{N}(e_t)$}
{
	$M' = Match(e_t) \times Match(e_{t'}) \cap \trans{E}_q$ \\
	\ForEach{$(e_{q_1}, e_{q_2}) \in M'$}
	{
		\If{$(e_t, e_{t'})$ comparable with $(e_{q_1}, e_{q_2})$}
		{
			Add edge $(e_t, e_{t'})$ into $\trans{E}$ if not exist  \\
			/* label of edges in $\trans{E}$ is a set of ids */ \\
			$\trans{L}(e_t, e_{t'}).add(ID_{{q_1}{q_2}})$
		}
	}
}
RETURN \\
\end{algorithm}

\begin{algorithm}[t]
\small
\caption{Explore($e_t$, $E_m$)}
 \label{alg:explore}
\KwIn{A new edge $e_t$ in $E_q$}
\KwOut{Output all new matching subgraphs}
\If{$E_m = \emptyset$}
{
	\ForEach{$e_q \in Match(e_t)$}
	{
		$vec[e_q] = e_t$\ \  /*match $e_q$ with $e_t$*/ \\
		Update the two vector $Tmax[]$ and $Tmin[]$ \\
		$E_m.add(e_q)$ \\		
		Initial $\N(E_m)$ with $\N(e_q)$\ \ /* $\N(E_m) = E_m\times (E_q - E_m) \cap \trans{E}_q$  */ \\
		$Explore(e_t, E_m)$ \\
		Restore data structure \\
	}
	RETURN
}
\If{$\N(E_m) = \emptyset$}{
	$Output(vec)$\ \ /*output matching subgraph*/
}
\Else
{
	\ForEach{$(e_{q_1}, e_{q_2}) \in \N(E_m)$}{
		let $e_{t_1} = vec[e_{q_1}]$  \\
		\ForEach{$e_{t_2} \in \trans{N}(e_{t_1})$ where $ID_{q_1q_2} \in$ $\trans{L}((e_{t_1}, e_{t_2}))$}
		{
			\If{$verify(vec, e_{q_2}, e_{t_2}) = TRUE$}{
				$vec[e_{q_2}] = e_{t_2}$ \\
				Update the two vector $Tmax[]$ and $Tmin[]$ \\
				$E_m.add(e_q)$ \\
				Update $\N(E_m)$ \\
				
			}
			Restore data structure\textbf{}
		}  

	}
}
RETURN \\
\end{algorithm}


} % nop

==> relatedwork.tex <==
\vspace{-0.1in}
\section{Related Work}
\vspace{-0.05in}
\label{sec:relatedwork}
%PART1 subgraph search(), most static(), ullman, vf2, matrix... ++ continous
Subgraph search has been extensively studied (e.g., \cite{vf2cordella2001improved,vf2TKDBcordella2004sub,sgi-planar-eppstein1995subgraph,sgi-closure2006he,sgi-krissinel2004common,sgi-messmer1998new,ullmann1976algorithm}) with the focus predominantly on static graph data. There are two popular subgraph isomorphism algorithms: Ullman \cite{ullmann1976algorithm} proposes a well-known subgraph isomorphism algorithm that is based on a state-space search approach; Cordella et al. \cite{vf2cordella2001improved} propose the VF2 algorithm that employs a filtering and verification strategy and outperforms Ullman's algorithm. % illustrate more on static technique: indexing, filtering

%PART2 continuous(), Fan, Chen, Gao, Event, SJ-tree, two close works
\vspace{-0.15in}
\begin{table}[!h]
\centering
\caption{Related work VS. Our Method}     % NOTE!  caption goes _before_ the table contents !!
\label{tab:relatedwork}
\resizebox{\linewidth}{!}{
  \input{tab/tab_relatedwork}
}
\end{table}
\vspace{-0.1in}
The research on continuous query processing over high-speed streaming graph data has recently started to attract attention. 
% challenge
Fan et al. \cite{fan2013incremental} propose an incremental solution for subgraph isomorphism based on repeated search over dynamic graph data, which cannot utilize previously computed results when new data come from the stream since they do not maintain any partial result. To avoid the high overhead in building complicated index, there is some work on approximate solution to subgraph isomorphism. 
% Chen et al.  
Chen et al. \cite{chen2010continuous} propose \emph{node-neighbor tree} data structure to search multiple graph streams; they relax the exact match requirement and their solution needs to conduct significant processing on the graph streams. Also, graph stream in \cite{chen2010continuous} is a sequence of small data graphs, which is not our focus.
% Gao et al.
Gao et al. \cite{gao2014continuous} study continuous subgraph search over a graph stream. They make specific assumption over their query and their solution cannot guarantee exact answers for subgraph isomorphism.
% event pattern
Song et al. \cite{eventpatternmatching14song} is the first work to impose timing order in subgraph simulation, a kind of loose subgraph search losing topology of the query compared with subgraph isomorphism. They verify the timing order over candidate answers after they retrieve them instead of utilizing the important timing order feature in the streaming data to accelerate the corresponding computation. 
% sj-tree
Choudhury et al. \cite{selectivityedbt15} study subgraph isomorphism over streaming graph without timing constraints. In other words, they only consider the \emph{structure constraint} and ignore the \emph{timing order constraint}. They propose a subgraph join tree (SJ-tree) to maintain some intermediate results, where the root contains answers for the query while the other nodes store partial matches. Their solution suffers from large space usage due to maintaining results. Ours is the first proposal to compute subgraph isomorphism over streaming graph with partial timing order constraints. Table \ref{tab:relatedwork} summarizes the differences between our method with other work on continuous subgraph search. In our solution, we propose match-store tree (MS-tree) to greatly reduce the space redundancy and accelerate the deletion operations for expired edges.

%PART3 solution similarity with SJ-tree, comparison

%PART4 conclusion, none of both timing+subgraph isomorphism, MS-tree, parallel(acceleration+without huge communication in distributed setting)





==> wiki-talk.tex <==
\begin{figure}[h!]
\centering
    %=========================================win-wkt
    \begin{subfigure}[t]{0.45\linewidth}
	    \centering
	    \resizebox{\linewidth}{!}
	    {
	        \includegraphics{\timefolder time_win_wkt.pdf}
	    }
	    \caption{Varying Window Size}
	    \label{res-fig:time:win:wkt}
    \end{subfigure}
      	\hspace{0.1in} 
    %=========================================rdf
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \resizebox{\linewidth}{!}
        {
            \includegraphics{\timefolder time_qsz_wkt.pdf}
        }
        \caption{Varying Query Size}
        \label{res-fig:time:qsz:wkt}
    \end{subfigure}
     %=========================================wkt
\caption{Throughput over Wiki-talk}
\label{res-fig:time:wkt}
\end{figure}

\begin{figure}[h!]
\centering
    %=========================================win-wkt
    \begin{subfigure}[t]{0.45\linewidth}
	    \centering
	    \resizebox{\linewidth}{!}
	    {
	        \includegraphics{\spacefolder space_win_wkt.pdf}
	    }
	    \caption{Varying Window Size}
	    \label{res-fig:space:win:wkt}
    \end{subfigure}
      	\hspace{0.1in} 
    %=========================================rdf
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \resizebox{\linewidth}{!}
        {
            \includegraphics{\spacefolder space_qsz_wkt.pdf}
        }
        \caption{Varying Query Size}
        \label{res-fig:space:qsz:wkt}
    \end{subfigure}
     %=========================================wkt
\caption{Space over Wiki-talk}
\label{res-fig:space:wkt}
\end{figure}

\begin{figure}[h!]
\centering
    %=========================================win-wkt
    \begin{subfigure}[t]{0.45\linewidth}
	    \centering
	    \resizebox{\linewidth}{!}
	    {
	        \includegraphics{\spdfolder spd_win_wkt.pdf}
	    }
	    \caption{Varying Window Size}
	    \label{res-fig:spd:win:wkt}
    \end{subfigure}
      	\hspace{0.1in} 
    %=========================================rdf
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \resizebox{\linewidth}{!}
        {
            \includegraphics{\spdfolder spd_qsz_wkt.pdf}
        }
        \caption{Varying Query Size}
        \label{res-fig:spd:qsz:wkt}
    \end{subfigure}
     %=========================================wkt
\caption{Speedup over Wiki-talk}
\label{res-fig:spd:wkt}
\end{figure}
